PhyMo: A Physical-Field Modality for Multimodal AI4Physics

Multimodal learning is emerging as a powerful paradigm for AI for Physics (AI4Physics), where predicting physical systems requires the joint interpretation of heterogeneous observations, measurements, and domain knowledge. However, existing approaches typically represent physical quantities and governing equations as generic numerical or textual tokens, overlooking the physical constraints that determine their spatiotemporal interactions. To address this limitation, we introduce the \textbf{physical-field modality} and propose \textbf{PhyMo}, a physics-grounded multimodal framework that organizes heterogeneous measurements through PDE-associated operators. PhyMo follows a three-stage learning procedure: the physical-field encoder is first pretrained through field reconstruction under PDE residual supervision, its representations are subsequently aligned with visual embeddings in a shared latent space, and the fused multimodal representations are finally processed by corresponding downstream prediction heads. Experiments on five datasets spanning diverse physical environments show that PhyMo achieves state-of-the-art performance, compared to the strongest baseline on each dataset, demonstrating the superiority of PhyMo on multimodal representation learning in AI4Physics.

==> ablation_r2_table_skippd.tex <==
% Requires: \usepackage{booktabs}
% Optional: \usepackage{microtype}
\begin{table}[t]
\centering
\caption{Ablation analysis of the proposed model on the SKIPP'D test set.
Each entry is the mean $R^2$ $\pm$ sample standard deviation over five outer
seeds; higher $R^2$ is better. Bold denotes the best mean within each
experiment.}
\label{tab:ablation-r2-skippd}
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.18}
\footnotesize
\begin{tabular}{@{}lllc@{}}
\toprule
Experiment & Setting & Configuration & \shortstack{SKIPP'D\\$R^2$}\\
\midrule
Modality & Both & Both modalities & 0.8470 $\pm$ 0.0021 \\
& w/o field & Field modality removed & \textbf{0.8490 $\pm$ 0.0021} \\
& w/o image & Image modality removed & 0.8345 $\pm$ 0.0014 \\
\addlinespace[2pt]
Fusion & EF & Early fusion & \textbf{0.8480 $\pm$ 0.0014} \\
& LF & Strict late fusion & 0.8480 $\pm$ 0.0013 \\
\bottomrule
\end{tabular}

\vspace{0.25em}
\parbox{0.98\linewidth}{\footnotesize\emph{Notes.} Results are evaluated at
$H=15$ min. In the modality ablation, deleting a modality removes its encoder
and corresponding data inputs, and every arm omits the Stage-2 adapter. EF
retains the joint Stage-1 Transformer and Stage-2 adapter, whereas LF uses
independent Stage-1 streams and removes Stage 2. Boldface is descriptive and
does not imply statistical significance.}
\end{table}


==> experiments_table.tex <==
% Requires: \usepackage{booktabs}
% Requires: \usepackage{graphicx}
% Optional: \usepackage{microtype}
\begin{table*}[t]
\centering
\caption{Experimental results across datasets. Each entry is the mean $R^2$ $\pm$ sample standard deviation over five outer seeds, expressed in percentage points with the percent sign omitted. For each dataset, we bold the model with the best performance.}
\label{tab:sheet1-r2}
\setlength{\tabcolsep}{1.4pt}
\renewcommand{\arraystretch}{1.05}
\scriptsize
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l*{15}{c}@{}}
\toprule
Dataset & Lasso & Ridge & RF & LSTM & ResNet-50 & TabM & TSMixer & RealMLP & ModernNCA & xLSTM & BiMamba & AstroCLIP & Maven & AION-1 & \textbf{Ours} \\\\
\midrule
SKIPP'D & 82.61$\pm$0.00 & 82.86$\pm$0.00 & 83.44$\pm$0.03 & 83.65$\pm$0.48 & 82.65$\pm$0.37 & 83.82$\pm$0.26 & 83.69$\pm$0.42 & 83.75$\pm$0.71 & 82.46$\pm$1.13 & 83.65$\pm$0.30 & 83.13$\pm$0.56 & 82.62$\pm$0.31 & 75.86$\pm$1.68 & 77.94$\pm$1.55 & \textbf{84.80$\pm$0.14} \\\\
Folsom & 94.44$\pm$0.00 & 94.35$\pm$0.00 & 95.27$\pm$0.00 & 95.17$\pm$0.03 & 94.08$\pm$0.01 & 95.21$\pm$0.02 & 95.18$\pm$0.02 & 95.21$\pm$0.01 & 94.84$\pm$0.01 & 95.17$\pm$0.02 & 95.18$\pm$0.03 & 94.63$\pm$0.03 & 92.19$\pm$0.09 & 94.44$\pm$0.03 & \textbf{95.35$\pm$0.03} \\\\
NREL & 73.40$\pm$0.00 & 73.40$\pm$0.00 & 74.98$\pm$0.01 & 77.37$\pm$0.03 & 69.65$\pm$0.17 & 76.23$\pm$0.02 & 75.50$\pm$0.04 & 76.32$\pm$0.01 & 74.28$\pm$0.13 & 77.33$\pm$0.08 & 77.33$\pm$0.06 & 77.38$\pm$0.03 & 72.67$\pm$0.50 & 73.72$\pm$0.21 & \textbf{79.31$\pm$0.26} \\\\
MeteoNet & 96.38$\pm$0.00 & 96.38$\pm$0.00 & 93.38$\pm$0.06 & 97.65$\pm$0.06 & 91.87$\pm$0.69 & 97.61$\pm$0.04 & 97.64$\pm$0.01 & 97.67$\pm$0.02 & 96.10$\pm$0.44 & \textbf{97.78$\pm$0.01} & 97.76$\pm$0.03 & 97.45$\pm$0.03 & 91.23$\pm$0.58 & 93.81$\pm$0.22 & 97.36$\pm$0.07 \\\\
Boreas & 99.08$\pm$0.00 & 99.08$\pm$0.00 & 13.11$\pm$5.23 & 92.77$\pm$5.98 & 93.38$\pm$2.49 & 96.95$\pm$2.82 & 96.48$\pm$1.85 & 98.65$\pm$0.23 & 72.49$\pm$20.49 & 99.07$\pm$0.23 & \textbf{99.24$\pm$0.25} & 38.81$\pm$11.55 & 29.01$\pm$2.71 & -60.59$\pm$6.99 & 90.49$\pm$4.28 \\\\
\bottomrule
\end{tabular}
}
\end{table*}


==> hyperparam_sensitivity_table.tex <==
% Requires: \usepackage{booktabs}
% Requires: \usepackage{graphicx}
% Optional: \usepackage{microtype}
\begin{table}[t]
\centering
\caption{Sensitivity analysis of the proposed model on the SKIPPD test set. Each entry is the mean $R^2$ $\pm$ sample standard deviation over five outer seeds; higher $R^2$ is better. Bold denotes the best mean within each horizon column.}
\label{tab:hyperparam-sensitivity}
\setlength{\tabcolsep}{3.4pt}
\renewcommand{\arraystretch}{1.15}
\footnotesize
\newcommand{\rstd}[2]{\mbox{$#1_{\pm #2}$}}
\newcommand{\brstd}[2]{\mbox{\boldmath$#1_{\pm #2}$}}

\begin{minipage}[t]{0.492\linewidth}
\centering
\textbf{(a) Stage 1 supervision horizon (SKIPPD)}\par\vspace{2pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}llccccc@{}}
\toprule
Setting & \shortstack{Supervision set\\(min)} & H15 & H30 & H60 & H120 & Mean \\
\midrule
K1 & $\{5\}$ & \rstd{0.8465}{0.0028} & \rstd{0.8069}{0.0036} & \rstd{0.7707}{0.0047} & \rstd{0.7089}{0.0055} & \rstd{0.7832}{0.0034} \\
K2 & $\{5,15\}$ & \rstd{0.8485}{0.0027} & \rstd{0.8057}{0.0028} & \rstd{0.7675}{0.0078} & \brstd{0.7123}{0.0076} & \rstd{0.7835}{0.0047} \\
K3 & $\{5,15,30\}$ & \rstd{0.8477}{0.0020} & \brstd{0.8085}{0.0023} & \brstd{0.7707}{0.0035} & \rstd{0.7107}{0.0071} & \brstd{0.7844}{0.0030} \\
K4 & $\{5,15,20,30\}$ & \brstd{0.8494}{0.0009} & \rstd{0.8081}{0.0018} & \rstd{0.7699}{0.0048} & \rstd{0.7067}{0.0059} & \rstd{0.7835}{0.0024} \\
K6 & $\{5,10,15,20,25,30\}$ & \rstd{0.8490}{0.0025} & \rstd{0.8051}{0.0046} & \rstd{0.7694}{0.0059} & \rstd{0.7115}{0.0065} & \rstd{0.7838}{0.0044} \\
\bottomrule
\end{tabular}%
}
\end{minipage}%
\hfill
\begin{minipage}[t]{0.492\linewidth}
\centering
\renewcommand{\arraystretch}{0.985}
\textbf{(b) Stage 3 historical-image span (SKIPPD)}\par\vspace{2pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}llccccc@{}}
\toprule
Setting & \shortstack{Span\\(frames)} & H15 & H30 & H60 & H120 & Mean \\
\midrule
C5 & 6 & \brstd{0.8496}{0.0018} & \rstd{0.8078}{0.0021} & \brstd{0.7735}{0.0048} & \brstd{0.7148}{0.0047} & \brstd{0.7865}{0.0029} \\
C15 & 16 & \rstd{0.8480}{0.0014} & \brstd{0.8086}{0.0027} & \rstd{0.7703}{0.0048} & \rstd{0.7133}{0.0101} & \rstd{0.7851}{0.0019} \\
C30 & 31 & \rstd{0.8488}{0.0023} & \rstd{0.8082}{0.0031} & \rstd{0.7689}{0.0037} & \rstd{0.7143}{0.0090} & \rstd{0.7851}{0.0041} \\
C45 & 46 & \rstd{0.8475}{0.0019} & \rstd{0.8065}{0.0040} & \rstd{0.7648}{0.0076} & \rstd{0.7057}{0.0069} & \rstd{0.7811}{0.0037} \\
C60 & 61 & \rstd{0.8450}{0.0011} & \rstd{0.8048}{0.0023} & \rstd{0.7652}{0.0024} & \rstd{0.7110}{0.0092} & \rstd{0.7815}{0.0021} \\
\bottomrule
\end{tabular}%
}
\end{minipage}

\vspace{0.8em}
\begin{minipage}[t]{\linewidth}
\centering
\textbf{(c) Cross-modal embedding size (SKIPPD)}\par\vspace{2pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}rcccccc@{}}
\toprule
EMB & Rep. width & H15 & H30 & H60 & H120 & Mean \\
\midrule
64 & 192 & \rstd{0.8461}{0.0015} & \rstd{0.8083}{0.0031} & \rstd{0.7710}{0.0040} & \rstd{0.7147}{0.0076} & \rstd{0.7850}{0.0031} \\
96 & 288 & \rstd{0.8480}{0.0014} & \rstd{0.8080}{0.0016} & \rstd{0.7706}{0.0033} & \brstd{0.7168}{0.0022} & \brstd{0.7858}{0.0013} \\
128 & 384 & \rstd{0.8480}{0.0014} & \rstd{0.8086}{0.0025} & \rstd{0.7708}{0.0055} & \rstd{0.7130}{0.0102} & \rstd{0.7851}{0.0021} \\
160 & 480 & \rstd{0.8469}{0.0017} & \rstd{0.8051}{0.0035} & \rstd{0.7696}{0.0027} & \rstd{0.7101}{0.0044} & \rstd{0.7829}{0.0017} \\
192 & 576 & \rstd{0.8490}{0.0006} & \brstd{0.8103}{0.0023} & \brstd{0.7725}{0.0051} & \rstd{0.7067}{0.0050} & \rstd{0.7846}{0.0024} \\
256 & 768 & \brstd{0.8495}{0.0020} & \rstd{0.8074}{0.0018} & \rstd{0.7716}{0.0027} & \rstd{0.7104}{0.0052} & \rstd{0.7847}{0.0026} \\
\bottomrule
\end{tabular}%
}
\end{minipage}

\vspace{0.35em}
\parbox{\linewidth}{\scriptsize\emph{Notes.} In all panels, each horizon cell is the mean over five outer seeds, and the reported mean is the equal-weight mean over H15, H30, H60 and H120 computed per seed before aggregation. Stage 1 changes only the supervised future-image horizon set. Stage 3 uses a fixed 1-min image cadence and changes only historical span (6, 16, 31, 46 and 61 frames). All runs use EMB=128 except panel (c).}
\end{table}

